Retinex-based Image Denoising / Contrast Enhancement using Gradient Graph Laplacian Regularizer

Images captured in poorly lit conditions are often corrupted by acquisition noise. Leveraging recent advances in graph-based regularization, we propose a fast Retinex-based restoration scheme that denoises and contrast-enhances an image. Specifically, by Retinex theory we first assume that each image pixel is a multiplication of its reflectance and illumination components. We next assume that the reflectance and illumination components are piecewise constant (PWC) and continuous piecewise planar (PWP) signals, which can be recovered via graph Laplacian regularizer (GLR) and gradient graph Laplacian regularizer (GGLR) respectively. We formulate quadratic objectives regularized by GLR and GGLR, which are minimized alternately until convergence by solving linear systems -- with improved condition numbers via proposed preconditioners -- via conjugate gradient (CG) efficiently. Experimental results show that our algorithm achieves competitive visual image quality while reducing computation complexity noticeably.

==> result_tables.tex <==
\begin{table}[!htbp]
\centering
\caption{Computation complexity comparison of LR3M \cite{ren20} and our method based on running time in seconds.}
\label{tab:comparison}
\vspace{-0.05in}
\begin{footnotesize}
\begin{tabular}{llrr}
\hline
Image        & Resolution       & LR3M \cite{ren20} & Ours  \\ \hline
\texttt{Moonlight}    & $560 \times 420$ & 250.48            & \textbf{25.17} \\
\texttt{Cars}         & $370 \times 415$ & 284.00            & \textbf{16.24} \\
\texttt{Plant}        & $500 \times 375$ & 142.08            & \textbf{21.91} \\
\texttt{Bear}         & $490 \times 365$ & 162.24            & \textbf{20.82} \\
\texttt{Nightfall}    & $690 \times 460$ & 301.75            & \textbf{35.20} \\
\texttt{Street}       & $1035 \times 785$ & 1442.23           & \textbf{88.24} \\
\texttt{Stormtrooper} & $450 \times 450$ & 87.36             & \textbf{21.09} \\
\texttt{Riverside}    & $720 \times 680$ & 366.41            & \textbf{52.82} \\
\texttt{Landmark}     & $540 \times 720$ & 148.01            & \textbf{42.59} \\
\texttt{Man}          & $895 \times 590$ & 246.40            & \textbf{56.47} \\
\texttt{Lamp}         & $450 \times 500$ & 165.40            & \textbf{24.37} \\
\texttt{Wire}         & $325 \times 325$ & 152.29            & \textbf{11.92} \\ \hline
\multicolumn{2}{r}{Average} & 310.92 & \textbf{32.43} \\ \hline
\end{tabular}
\end{footnotesize}
\end{table}

\begin{table*}[!htbp]
\centering
\caption{MDM score.}
\label{tab:comparison}
\vspace{-0.05in}
\begin{footnotesize}
\begin{tabular}{l|c|c|c|c|c|c}
\hline
Image        & Noisy image       & Model from \cite{DBLP:conf/cvpr/FuZHZD16}        & LIME \cite{DBLP:journals/tip/GuoLL17} & JED \cite{DBLP:journals/corr/abs-1804-08468} & {LR3M \cite{ren20}} & \multicolumn{1}{c}{Ours}  \\ \hline
\texttt{Moonlight}    & 0.9594 & 0.9522            & \textbf{0.9683} & 0.9652 & \textbf{0.9672}             & 0.9663 \\
\texttt{Cars}         & 0.9611 & 0.9440            & \textbf{0.9553} & 0.9483 & 0.9514             & \textbf{0.9578} \\
\texttt{Plant}        & 0.9633 & 0.9582            & \textbf{0.9748} & 0.9709 & \textbf{0.9739}             & 0.9726 \\
\texttt{Bear}         & 0.8384 & 0.9076            & \textbf{0.9760} & 0.9750 & \textbf{0.9756}             & 0.9716 \\
\texttt{Nightfall}    & 0.9711 & 0.9643            & \textbf{0.9763} & 0.9735 & \textbf{0.9767}             & 0.9741 \\
\texttt{Street}       & 0.9706 & 0.9682           & 0.9762 & \textbf{0.9785} & \textbf{0.9767}             & 0.9754 \\
\texttt{Stormtrooper} & 0.9689 & 0.9612             & 0.9745 & 0.9716 & \textbf{0.9752}             & \textbf{0.9760} \\
\texttt{Riverside}    & 0.9707 & 0.9589            & \textbf{0.9758} & 0.9721 & 0.9707             & \textbf{0.9739} \\
\texttt{Landmark}     & 0.9571 & 0.9435            & \textbf{0.9613} & 0.9465 & 0.9515             & \textbf{0.9601} \\
\texttt{Man}          & \textbf{0.9372} & \textbf{0.9243}            & 0.9176 & 0.9107 & 0.9048             & 0.9224 \\
\texttt{Lamp}         & 0.9702 & 0.9612            & \textbf{0.9733} & \textbf{0.9721} & 0.9709             & 0.9705 \\
\texttt{Wire}         & 0.9634 & 0.9575            & \textbf{0.9782} & 0.9770 & \textbf{0.9782}             & 0.9729 \\ \hline
{Average} & 0.9526 & 0.9501 & \textbf{0.9673} & 0.9635 & 0.9644 & \textbf{0.9661} \\ \hline
\end{tabular}
\end{footnotesize}
\end{table*}


\begin{table}[htbp]
\centering
\caption{LOE score.}
\label{tab:comparisonLOE}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Image        & M1 \cite{DBLP:conf/cvpr/FuZHZD16}        & LIME \cite{DBLP:journals/tip/GuoLL17} & JED \cite{DBLP:journals/corr/abs-1804-08468} & LR3M \cite{ren20} & Ours \\ \hline
\texttt{Mnl} & 0.6185 & \textbf{0.5444} & 1.0730 & 0.9590 & \textbf{0.4817} \\
\texttt{Crs} & 0.5887 & 0.7051 & 1.0487 & 1.0257 & \textbf{0.5479} \\
\texttt{Plt} & 0.8414 & \textbf{0.703}  & \textbf{0.6998} & 0.8754 & 0.8006 \\
\texttt{Ber} & 0.8517 & \textbf{0.6703} & 0.9291 & 1.3507 & \textbf{0.7682} \\
\texttt{Nfl} & 0.8879 & 0.7364 & \textbf{0.4850} & 0.7349 & \textbf{0.4701} \\
\texttt{Str} & \textbf{0.6415} & \textbf{0.5858} & 0.7661 & 1.2604 & 0.7317 \\
\texttt{Strp} & 0.9141 & \textbf{0.7486} & 1.2178 & 0.8096 & \textbf{0.6590} \\
\texttt{Rvs} & 0.9684 & \textbf{0.6977} & 0.7341 & 1.1203 & \textbf{0.5003} \\
\texttt{Lmk} & 0.8279 & \textbf{0.6800} & 1.0666 & 0.8346 & \textbf{0.5080} \\
\texttt{Man} & \textbf{0.6675} & 0.8141 & 0.8456 & 1.2376 & \textbf{0.5209} \\
\texttt{Lmp} & \textbf{0.6135} & \textbf{0.5644} & 1.1641 & 1.9776 & 0.7960 \\
\texttt{Wir} & \textbf{0.6875} & \textbf{0.6515} & 1.2575 & 1.4944 & 0.9911 \\ \hline
Avg & 0.7591 & \textbf{0.6751} & 0.9406 & 1.1400 & \textbf{0.6480} \\ \hline
\end{tabular}
\end{table}



\begin{table}[!htbp]
\centering
\caption{Quality comparison of comparing methods and our method based on LOE \cite{DBLP:journals/tip/WangZHL13} and MDM \cite{DBLP:journals/tbc/NafchiC18} score.}
\label{tab:comparison}
\vspace{-0.05in}
\begin{footnotesize}
\begin{tabular}{l|cc}
\hline
Image        & Avg. LOE & Avg. MDM \\ \hline
Model from \cite{DBLP:conf/cvpr/FuZHZD16}    & 0.7591 & 0.9501\\
LIME \cite{DBLP:journals/tip/GuoLL17}       & 0.6751 & \textbf{0.9673} \\
JED \cite{DBLP:journals/corr/abs-1804-08468}        & 0.9406 & 0.9635       \\
LR3M \cite{ren20}         &  1.1400 & 0.9644\\
Ours    & \textbf{0.6480} & 0.9661 \\\hline
\end{tabular}
\end{footnotesize}
\end{table}

